Mint: MDL-based approach for Mining INTeresting Numerical Pattern Sets

Pattern mining is well established in data mining research, especially for mining binary datasets. Surprisingly, there is much less work about numerical pattern mining and this research area remains under-explored. In this paper, we propose Mint, an efficient MDL-based algorithm for mining numerical datasets. The MDL principle is a robust and reliable framework widely used in pattern mining, and as well in subgroup discovery. In Mint we reuse MDL for discovering useful patterns and returning a set of non-redundant overlapping patterns with well-defined boundaries and covering meaningful groups of objects. Mint is not alone in the category of numerical pattern miners based on MDL. In the experiments presented in the paper we show that Mint outperforms competitors among which Slim and RealKrimp.

==> old_rw.tex <==


\section{Introduction}

Pattern Mining (PM) is an umbrella that encompasses a large variety of methods, processes, and algorithms of Knowledge Discovery and Data Mining aimed at getting insight from data. 
The goal of PM is to discover a small set of interesting patterns that describe together a large portion of data and can be easily interpreted by humans. 

The modern approaches to PM are aimed to find an interesting \textit{pattern set} rather than a set of individually interesting patterns, i.e., the quality of patterns is evaluated w.r.t. both the dataset and other patterns. 
One of the most commonly used theoretical basis for pattern set mining is the Minimum Description Length principle (MDL)~\cite{grunwald2007minimum}. 
It was applied to a large variety of patterns: itemsets~\cite{vreeken2011krimp}, patterns of arbitrary shapes in 2-dimensional data~\cite{faas2020vouw}, sequences~\cite{hinrichs2017characterising}, graphs~\cite{bariatti2020graphmdl}.

Despite the recent advances in PM, the methods for mining numerical data remain insufficiently explored. 
To date, one of the most common way to mine numerical pattern sets remains itemset mining applied to binarized dataset.
We discuss the approaches to numerical PM in detail in the next section. 

An alternative to numerical PM is clustering. 
For the last decades, clustering approaches have been extensively developed, and a large amount of different efficient approaches have been proposed. 
However, there is an important, rather conceptual, difference between PM and clustering. 
In PM the \textit{description} comes first, while in clustering the primacy is given to the object similarity. In other words, patterns are considered as some subspaces in the attribute space. 
The latter entails requirements for ease of interpretation, i.e., the obtained patterns should describe the corresponding region in the attribute space in such a way to ensure a simple interpretation by humans.

In clustering, on the contrary, we are interested in \textit{instances} that are grouped together. 
The shapes of clusters can also be restricted to certain shapes, e.g., spheres in Kmeans or DBScan, but still the similarity of objects remains the most important characteristic of clusters.
For example, such clustering techniques as agglomerative single-linkage clustering in multidimensional space may return clusters of very complex shapes, and usually no attention is paid to shapes of such clusters.

In this study, we propose an MDL-based approach to numerical pattern set mining called \textsc{Mint} for ``Mining INTeresting Numerical Pattern Sets''. 
It computes numerical patterns as $m$-dimensional hyper-rectangles, i.e., products of $m$ intervals.
The main benefits of the \textsc{Mint} approach are that (i) \textsc{Mint} does not imply exploring pattern space in advance, candidates to optimal patterns are computed on the fly, (ii) the total number of explored patterns is at most quadratic in the number of objects with distinct descriptions (vectors of attribute values), (iv) \textsc{Mint} is based on MDL, i.e., the result consists of a small set of non-redundant informative patterns.

The paper has the following structure. 
In Section~\ref{sec:related_work} we discuss the state-of-the art methods for quantitative itemset pattern mining.
Section~\ref{sec:basics} introduces the main notions used in the paper. 
In Section~\ref{sec:method} we describe the proposed method. 
Section~\ref{sec:experiments} contains the results of the experiments. 
In Section~\ref{sec:conclusion} we conclude and give possible directions for future work.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Numerical Pattern Mining envelops a large variety of methods, techniques, and even types of patterns. 
The problem of PM has been extensively studied for binary data (in Itemset Mining), however remains almost unexplored for numerical data. 
The most common way to mine patterns in numerical data is to binarize it and then apply a method for Itemset Mining.

In this section we firstly discuss different data preprocessing approaches used to apply IM methods to numerical data, and then discuss the state-of-the art approaches in PM.

\subsection{Data Preprocessing}

Application of itemset mining methods to binarized data is considered to be the most common way to mine numerical patterns. 
These approaches are usually referred to as quantitative itemset mining~\cite{srikant1996mining}. 
In quantitative itemset mining, data preprocessing is the cornerstone for getting good-quality patterns. 
The preprocessing can be decomposed into \textit{discretization} and \textit{binarization}.  

\subsubsection{Discretization}
Discretization --partitioning a range of attribute values into intervals, and mapping the intervals into integers
preserving the order of the intervals-- is one of the most challenging steps in numerical PM. 
The existing discretization techniques can be categorized into two classes: \textit{univariate} and \textit{multivariate}. Here, we consider only techniques applicable in unsupervised settings.

The univariate discretization includes all the methods where attributes are considered independently. 
The most common approaches are splitting an attribute range into intervals of equal-width or equal-height (frequency). 
Another widely used method consists in splitting each attribute range based on $K$-means algorithm~\cite{dash2011comparative}, where some standard criteria for assessing quality of clustering can be used to choose an optimal $K$. 
A more flexible approach consists in splitting based on the MDL principle~\cite{kontkanen2007mdl,rissanen1992density}. 

Considering each attribute range independently, the aforementioned approaches do not preserve interaction between attributes, and as a consequence, can make some patterns unrecognizable.

The multivariate discretization techniques were proposed to tackle this issue. In~\cite{mehta2005toward,kang2006ica} it was proposed to perform multivariate discretization based on Principal Component and Independent Component Analysis, respectively. 
However, both of them do not guarantee to identify complex interactions between attributes and require some assumption on either distribution or correlation~\cite{nguyen2014unsupervised}. 
In the same paper~\cite{nguyen2014unsupervised} the authors propose an MDL-method for multivariate discretization that does not have the above-mentioned shortcomings. 
Moreover, unlike its MDL-based cousin~\cite{fayyad93} this method works in unsupervised settings.

MDL has proven to be a powerful method for model selection: it is actively used in a wide range of tasks.
We go back later to it, just after the discussion of the data preprocessing approaches.

\subsubsection{Binarization}

Discretization is not the only step to accomplish before applying an itemset mining method. 
Another important question is binarization, i.e., transformation of discrete values into binary attributes. 
Even though usually little attention is paid to binarization, it may affect the results of Itemset Mining or cause loss of important information.

The simplest and most popular binarization strategy is one-hot encoding, where each discrete value is associated with one binary attribute. 
The number of attributes is large, which can lead to an excessive computational load. 
To mitigate the problem, similar and infrequent attributes can be removed. 
However for multidimensional data such a procedure usually does not solve the problem, i.e., the number of binary attributes becomes times as much as the number of attributes in the original dataset. 
Another drawback of one-hot encoding is that it does not preserve the order of discrete values. 
Moreover, this kind of discretization is very sensitive to very fine-scale discretization and completely unsuitable to the identification of patterns that are nested in the original data. 
Binarization is always associated with the risk of introducing artifacts and thus, obtaining meaningless results.

Interordinal scaling~\cite{kaytoue2011revisiting} appears to be less flawed than one-hot encoding. 
It preserves the order of values by introducing for each discrete value $v$ two binary attributes ``$x \geq v$'' and ``$x\leq v$''. 
However, in~\cite{kaytoue2011revisiting} it was shown that, with a low-frequency threshold, mining itemsets in interordinally scaled data becomes much more expensive than mining hyper-rectangles in numerical data. 

Therefore, despite of limitations of the one-hot encoding, it is given greater preference for reasons of an ``restrained'' attribute explosion, and more tractable computational costs.

\subsection{MDL-based approaches to PM}

In the previous section, we considered the common data preprocessing approaches applied to perform IM to numerical data. 
IM remains one of the most extensively studied fields of PM. 
(However, recently more complex patterns gain more and more popularity in scientific literature, e.g., graphs, sequences, etc.)

The recent IM approaches concern mining a pattern set rather than a set of patterns, i.e., computing the jointly interesting instead of individually interesting patterns.
One of the pioneers in this direction is~\cite{knobbe2006pattern}, where ``pattern teams'' were proposed. 
A pattern team is a set of patterns that are optimal w.r.t. several quality measures, including those that evaluate patterns w.r.t. other patterns. 
Although this method formalizes very intuitive ideas about the good properties of the pattern set, it may appear too handcrafted. 
Moreover, some of the proposed measures are applicable in supervised settings.

A move toward formal criterion for pattern sets was done in~\cite{chandola2007summarization}, where the authors use the measures of informativeness to find a small pattern set summarizing the whole dataset. 
In their work, they propose two measures: compaction gain and information loss. 
Broadly speaking, the compaction gain evaluates how typical a pattern for the dataset, while the information loss is used to control descriptiveness of itemsets w.r.t. the dataset. 
Put it differently, these two measures are used to find a model (set of patterns) that fits the data well but does not overfit it.

A significant stride in formalization of informativeness and finding a trade-off in the aforementioned problem was done by applying the MDL principle~\cite{grunwald2007minimum}. 
The MDL-based method works under the slogan: ``the best model is one that compresses given dataset best''.

One of the most famous MDL-based approached to IM was proposed in~\cite{vreeken2011krimp} and called \textsc{Krimp}. 
This is a two-step method that consists in (i) generating a set of frequent patters, (ii) and selecting those that minimize the total description length. 
The main drawback of \textsc{Krimp} is that it requires all frequent itemsets be generated. 
Moreover, increasing frequency threshold may result in worse compression. 

\textsc{Slim}~\cite{smets2012slim} was proposed to tackle this issue. 
This approach does not require all itemsets be generated in advance, the candidates to optimal itemsets are discovered gradually.  
However, the encoding scheme used in \textsc{Krimp} and \textsc{Slim} has a range of limitations (we postpone the details to Section~\ref{ssec:mdl}).

The \textsc{DiffNorm}~\cite{budhathoki2015difference} algorithm is an extension of the \textsc{Slim} that not only uses a better encoding scheme, but also is applicable to a set of datasets to find the difference in datasets in terms of itemsets. 

Another MDL method improving the scalability problem of \textsc{Krimp} was proposed in~\cite{akoglu2012fast}. 
This method deals with categorical data rather than with binary ones, thus less susceptible to attribute explosion due to fewer number of attributes.

All the aforementioned MDL-based methods represent a model --set of patterns-- as a two-column table, where the left-/right-hand columns contain the pattern descriptions and the associated code words, respectively. 
Another way to store patterns is used in \textsc{Pack} algorithms~\cite{tatti2008finding}. 
The model --set of patterns-- is encoded by means of a decision tree. 
In the decision tree, a node corresponds to an attribute. 
A non-leaf node has two siblings reflecting the presence or absence of this attribute in an itemset. 
The itemset, in turn, is a path from the root to a leaf node. The principle difference between \textsc{Pack} and \textsc{Krimp}-like methods is that in \textsc{Pack} 1s and 0s are treated symmetrically. 
%Geerts, F., Goethals, B., Mielik¨ainen, T.: Tiling Databases. In: Proc. DS, pp. 278–289 (2004)

Another representative of tree-based MDL approaches is \textsc{Stijl}~\cite{tatti2012style}. 
This approach also takes into account both 1s and 0s and store the itemsets in a tree, but this method is completely different from \textsc{Pack}. 
As patterns, this method uses tiles, i.e., rectangles in a dataset. 
Instead of the decision tree, the tree in \textsc{Stijl} is a hierarchy of nested tiles, where parent-child relations in the tree are inclusion relation in the set of tiles. 
A child tile is created if its density --the relative number of 1s-- differs a lot from the parent one.

The problem of tiles is closely related to Boolean Matrix Factorization. 
In a nutshell, the goal is find an approximation of a binary matrix $C$ by a Boolean product of two low-rank matrices $A$ and $B$. 
The columns of $A$ and the rows of $B$ describe the factors, which are tiles. 
The MDL priciple was also applied to the BMF problem~\cite{miettinen2014mdl4bmf,makhalova2020below}.

An extension (in a certain sense) of the tiling problem was introduced in~\cite{faas2020vouw} as geometric pattern mining problem. 
The authors consider arbitrarily shaped patterns in raster-based data, i.e., data tables with a fixed order of rows and columns. 
The proposed MDL-based approach, called \textsc{Vouw}, is able to identify descriptive pattern sets even in noisy data. 

All the considered above MDL-based methods deal with binary (or categorical). 
To date, there are a few approaches for mining patterns in numerical data. 

The \textsc{RealKrimp}~\cite{witteveen2014realkrimp} algorithm is an extension of \textsc{Krimp} for real-valued data. 
As patterns \textsc{RealKrimp} uses axis-aligned hyper-rectangles (i.e., boxes). 
The algorithm does not require any preprocessing, however, it discretizes the data under the hood. 
\textsc{RealKrimp} also does a feature selection by removing unimportant hyper-rectangle dimensions. 
The method is tailored to mine high-density patterns. 
To curb the pattern explosion, \textsc{RealKrimp} constructs a hyper-rectangle using a pair of the neighboring rows sampled from the original dataset. 
Thus, without prior knowledge about the data, the choice of the size of sampling is difficult: a too small sample size may results in very general patterns, while a too large sample size increases the execution time. 
The problem of inappropriate sample size may be partially solved by setting large \textit{perseverance}, i.e., how many closest rows should be checked to improve compression by enlarging the hyper-rectangle. 
Thus, the problem of finding an optimal parameters in \textsc{RealKrimp} becomes a part of the pattern mining process.
Another important characteristic of \textsc{RealKrimp} is that the hyper-rectangles are evaluated independently, meaning that instead of an optimal pattern set the algorithm searches for a set of optimal patterns. 
However, possible pattern redundancy can be mitigated by sampling data from different parts of the attribute space.
Thereby, working in very promising settings and having a strong mathematical foundation, \textsc{RealKrimp} has no means to evaluate jointly the set of generated hyper-rectangles and relies a lot on heuristics. 
The heuristics, in turn, imply some prior knowledge about the data, which are not always available in practice.

Another approach to mine informative hyper-rectangles in numerical data was proposed in~\cite{makhalova2019numerical}. 
The method can be summarized into 3 steps: (i) computing greedily dense hyper-rectangles by merging the closest neighbors and ranking them prioritizing dense regions, (ii) optimizing greedily an MDL-like objective to chose the intervals --sides of hyper-intervals-- for each attribute independently, (iii) constructing the patterns using chosen intervals and maximizing the number of instances described by the intervals (by applying the closure operator). 

However, the part (ii) lacks the strong formulation of the used MDL model. 
In fact, the method optimizes the entropy, which is proportional to the length of data encoded by the intervals, and does not take into account the complexity of the model, i.e., the set of patterns. 
This simplification is made based on the observation that each newly added interval replaces at least one of the existing, and thus, the complexity of the model does not increase. 
The used compression scheme is lossy, meaning that the data values can be reconstructed only up to chosen intervals. 
Like \textsc{RealKrimp}, it allows for feature selection and does not address the problem of overlapping patterns explicitly. 

In this study we propose an MDL-based approach called \textsc{Mint} to mining patterns in numerical data. 
As other methods we restrict the patterns to hyper-rectangles as the most interpretable types of multidimensional patterns. 
As \textsc{RealKrimp} our method deals with the discretized data, that allows us to define lossless compression scheme. 
We do not address the problem of the feature selection, however, allows patterns to overlap. 
Unlike its MDL-based cousin \textsc{RealKrimp}, our method search for an MDL-optimal pattern set rather that single patterns and is less dependent on heuristics. 


